Fractional vortex in asymmetric 0-$\pi$ long Josephson junctions

We consider an infinitely long 0-$\pi$ Josephson junction consisting of 0 and $\pi$ regions having different critical current densities $j_{c,0}$ and $j_{c,\pi}$. The ground state of such a junction corresponds to a spontaneosly formed asymmetric semifluxon with tails decaying on different length scales. We calculate the depinning current of such a fractional vortex and show that it is different for positive and negative bias polarity. We also show that upon application of a bias current, the fractional flux (topological charge) associated with the vortex changes. We calculate the range of fractional flux associated with the vortex when the bias changes from negative to positive critical (depinning) values.

==> MyMc.tex <==
%%% This is 'MyMc.tex' v3.00
%%% LaTeX macros for frequently used abbreviations
%%% 13.12.2011 by Edward Goldobin <gold@uni-tuebingen.de>

\RequirePackage{xspace}

%stupid macros like \ie, \eg, \etc
\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\vs}{\textit{vs.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\viz}{\textit{viz.}\xspace}
%\newcommand{\etal}{\textit{et~al.}\xspace}
\newcommand{\lhs}{l.h.s.\xspace}
\newcommand{\rhs}{r.h.s.\xspace}

\newcommand{\mum}{\ensuremath{\mathrm{\mu m}}}
\newcommand{\degree}{\ensuremath{^\circ}\xspace}

%units
\newcommand{\units}[1]{\ensuremath{\,\mathrm{#1}}}


% Convenient ratios and (partial) derivatives
%
%big \frac is called \ratio.
%usage: \ratio{a}{b}
\newcommand{\ratio}[2]{\displaystyle\frac{#1}{#2}}
%usage: \fracd{y}{x} produces fraction dy/dx.
%usage with optional argument: \fracd[2]{y}{x} produces 2nd derivative
\newcommand{\fracd}[3][]{\displaystyle\frac{d^{#1}#2}{d#3^{#1}}}
%usage: \fracp{y}{x} produces partial derivatice dy/dx.
%usage with optional argument: \fracp[2]{y}{x} produces 2nd order partial derivative
\newcommand{\fracp}[3][]{\displaystyle\frac{\partial^{#1}#2}{\partial#3^{#1}}}
%mixed derivatives are not implemented yet :-(

%Averaging macros:
%
%usage1: \av{V} - averaged V
%usage2: \av[x]{V} - V averaged with respect to x
\newcommand{\av}[2][]{\ensuremath{\left\langle#2\right\rangle}_{#1}\xspace}
%usage: \mean{u} - produced bar over the argument
\newcommand{\mean}[1]{\ensuremath{\overline{#1}}\xspace}
\newcommand{\dev}[2][]{\ensuremath{\widetilde{#2}_{#1}}\xspace}

%Freq used materials
\RequirePackage{xspace}
\newcommand{\YBCO}{YBa$_2$Cu$_3$O$_7$\xspace}
\newcommand{\LBCO}[1][x]{La$_{2-#1}$Ba$_#1$CuO$_4$\xspace}
\newcommand{\BSCCO}{Bi$_2$Sr$_2$Ca$_1$Cu$_2$O$_{8}$\xspace}
\newcommand{\NBCO}[1][x]{NdBa$_2$Cu$_3$O$_{7-#1}$\xspace}
\newcommand{\TBCO}{Tl$_2$Ba$_2$CuO$_6$\xspace}
\newcommand{\HBCO}{HgBa$_2$CuO$_6$\xspace}
\newcommand{\NCCO}{Nd$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\PCCO}{Pr$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\LCMO}[1][x]{La$_{1-#1}$Ca$_x$MnO$_3$\xspace}
\newcommand{\STO}{SrTiO$_3$\xspace}
\newcommand{\CeO}{CeO$_2$\xspace}
\newcommand{\MgB}{MgB$_2$\xspace}
\newcommand{\OrgIJJ}{$\kappa$-(BEDT-TTF)$_2$Cu(NCS)$_2$\xspace}


%technology definitions
\newcommand{\NbAlOxNb}{Nb-AlO$_x$-Nb\xspace}
\newcommand{\TechNb}{Nb-AlO$_x$-Nb\xspace}
\newcommand{\TechYBCONb}{YBCO-Nb\xspace}
%
\newcommand{\SIS}{\ensuremath{\mathrm{S|I|S}}\xspace}
\newcommand{\SNS}{\ensuremath{\mathrm{S|N|S}}\xspace}
\newcommand{\SFS}{\ensuremath{\mathrm{S|F|S}}\xspace}
\newcommand{\SIFS}{S$|$I$|$F$|$S\xspace}
\newcommand{\SfiS}{S$|$FI$|$S\xspace}
%\newcommand{\SJS}{\ensuremath{\mathrm{S-FI-S}}\xspace}

%%
%% Freq used math symbols
%%

%Elliptic fns
\newcommand{\am}{\mathop{\mathrm{am}}\nolimits}
\newcommand{\dn}{\mathop{\mathrm{dn}}\nolimits}
\newcommand{\sn}{\mathop{\mathrm{sn}}\nolimits}
\newcommand{\cn}{\mathop{\mathrm{cn}}\nolimits}
\newcommand{\gd}{\mathop{\mathrm{gd}}\nolimits}
\newcommand{\E} {\mathop{\mathrm{E}}\nolimits}
\newcommand{\F} {\mathop{\mathrm{F}}\nolimits}
\newcommand{\K} {\mathop{\mathrm{K}}\nolimits}
\newcommand{\J}[1][] {\mathop{\mathrm{J_{#1}}}\nolimits}
\newcommand{\Ai} {\mathop{\mathrm{Ai}}\nolimits}
\newcommand{\Bi} {\mathop{\mathrm{Bi}}\nolimits}

%Other fns
%\newcommand{\const}{\mathop{const}\nolimits}
\newcommand{\atanh}{\mathop{\mathrm{atanh}}\nolimits}
\newcommand{\acot}{\mathop{\mathrm{acot}}\nolimits}
\newcommand{\sech}{\mathop{\mathrm{sech}}\nolimits}
\newcommand{\sgn}{\mathop{\mathrm{sgn}}\nolimits}
\newcommand{\floor}{\mathop{\mathrm{floor}}\nolimits}
\newcommand{\const}{\mathop{\mathrm{const}}\nolimits}
\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}
%\newcommand{\Det}{\mathop{\mathrm{det}}\nolimits}
%\newcommand{\Tr}{\mathop{\mathrm{Tr}}\nolimits}

\newcommand{\qstate}[1]{\ensuremath{\left\lvert\state{#1}\right\rangle}}
\newcommand{\rot}{\mathop\mathrm{\mathbf{rot}}\nolimits}
\newcommand{\grad}{\mathop\mathbf{{\rm grad}}\nolimits}
%\newcommand{\div}{\mathop{{\rm div}}\nolimits}


%just shortcuts
%\newcommand{\HS}{\ensuremath{{\cal H}}}
\newcommand{\Heavyside}{\mathop{\mathrm{H}}\nolimits}
\newcommand{\G}{\ensuremath{{\cal G}}}
\newcommand{\Dx}{\ensuremath{{\Delta x}}}
\newcommand{\dx}{\ensuremath{{\delta x}}}
\newcommand{\Dw}{\ensuremath{{\Delta w}}}
\newcommand{\D}[1]{\ensuremath{{\Delta #1}}}
%\newcommand{\d}[1]{\ensuremath{{\delta #1}}}

%\iffalse%{
\RequirePackage{amssymb}

% macros for showing/hiding corrections

%\RequirePackage[normalem]{ulem}

%\newcommand{\new}[1]{\textcolor{blue}{#1}}
%\newcommand{\del}[1]{\textcolor{red}{\sout{#1}}}
%\newcommand{\chg}[1]{\textcolor{magenta}{#1}}
\RequirePackage{ifthen}
\newboolean{ShowCorrections}
\setboolean{ShowCorrections}{true}%<-- set here show/notshow corrections

%%%Reduction/Corrections macros
\ifthenelse{\boolean{ShowCorrections}}{%
\usepackage[normalem]{ulem}%
\newcommand{\new}[1]{\textcolor[rgb]{0,0,1}{#1}}%
\newcommand{\old}[1]{\textcolor[rgb]{1,0,0}{\sout{#1}}}%
}{%
\newcommand{\new}[1]{#1}%
\newcommand{\old}[1]{}%
}


%%
%% Not allowed stuff
%%

%state command which may not translate correctly
\newcommand{\stat}[1]{\state{#1}}

%%tth:\def\relax{}
%%tth:\def\message#1{}

%\tracingmacros=2
%%%%%%%%%%

\def\state#1{\ensuremath{\stt#1.}}
\def\stt#1{%
\if#1.
\let\next=\relax
\else
  \if#1u
    \upharpoonleft%\uparrow
  \else\if#1d
    \downharpoonleft%\downarrow
  \else\if#1U
    \upharpoonright%\Uparrow
  \else\if#1D
    \downharpoonright%\Downarrow
  \else\if#1F
    \Uparrow
  \else\if#1A
    \Downarrow
  \else\if#1s
    \uparrow
  \else\if#1a
    \downarrow
  \else\if#1r
    \rightarrow
  \else\if#1l
    \leftarrow
  \else\if#1R
    \Rightarrow
  \else\if#1L
    \Leftarrow
  \else\if#1>
    \longrightarrow
  \else\if#1<
    \longleftarrow
  \else\if#1
  \relax
  \else
  ?\message{Unknown symbol #1 in the argument of macro state}
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\let\next=\stt
\fi
\next
}

%usage: \hstruct{Nb|Al|Nb}
%at the moment cannot accept math or lower indices. :-(
\def\hstruct#1{%
\let\accu=\relax%
\hstruc#1.%
\accu
}
\def\hstruc#1{%
\if#1.%end?
\let\next=\relax
\else
  \if#1|%
    \let\accu=\accu$|$%
%  \else\if#1
%    \relax
  \else
    \let\accu=\accu #1%\message{Unknown symbol #1 in the argument of macro \hstruc}
  \fi%\fi
  \let\next=\hstruc
\fi
\next
}


\newcounter{CurrTimeHH}\newcounter{CurrTimeMM}
\newcommand{\CurrTime}{%
  \setcounter{CurrTimeHH}{\time/60}%
  \setcounter{CurrTimeMM}{\time - \value{CurrTimeHH}*60}%
  \ifthenelse{\value{CurrTimeHH}<10}{0}{}\theCurrTimeHH:%
  \ifthenelse{\value{CurrTimeMM}<10}{0}{}\theCurrTimeMM%
}




==> we.tex <==
%Misc. macros to discuss with co-authors
\RequirePackage{color}
\newcommand{\HS}[1]{{\textcolor{red}{\textbf{HS:``#1''}}}}
\newcommand{\EG}[1]{{\textcolor[rgb]{1,.4,0}{\textbf{EG:``#1''}}}}
\newcommand{\DK}[1]{{\textcolor[rgb]{0,0.7,0}{\textbf{DK:``#1''}}}}
\newcommand{\RK}[1]{{\textcolor[rgb]{1.0,0,0}{\textbf{RK:``#1''}}}}
\newcommand{\RM}[1]{{\textcolor[rgb]{0.4,.4,1}{\textbf{RM:``#1''}}}}

